Surfaces with maximal constant mean curvature

In this note we consider asymptotically flat manifolds with non-negative scalar curvature and an inner boundary which is an outermost minimal surface. We show that there exists an upper bound on the mean curvature of a constant mean curvature surface homologous to a subset of the interior boundary components. This bound allows us to find a maximizer for the constant mean curvature of a surface homologous to the inner boundary. With this maximizer at hand, we can construct an increasing family of sets with boundaries of increasing constant mean curvature. We interpret this familiy as a weak version of a CMC foliation.

==> argument.tex <==
\section{The Argument}
\label{sec:argument}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "master"
%%% End: 


==> extern/draft_commands.tex <==
\usepackage{ifthen}

%% Collect Time and Date Info
\makeatletter
\newcommand{\pt@twodigit}[1]{{\pt@tmp=#1\relax\ifnum\pt@tmp<10 0\fi\the\pt@tmp}}
\newcount\pt@hours
\newcount\pt@minutes
\newcount\pt@tmp
\newcommand{\printtime}{%
\pt@hours=\time%
\divide\pt@hours by 60\relax%
\pt@tmp=\pt@hours%
\multiply\pt@tmp by -60\relax%
\pt@minutes=\time%
\advance\pt@minutes by \pt@tmp%
\pt@twodigit\pt@hours:\pt@twodigit\pt@minutes}

%% How to put Info in the margin
\newlength{\mt@MarginWidth}
\newlength{\mt@PageHeight}
\newlength{\mt@ActualWidth}
\newlength{\mt@MaxWidth}
\newlength{\mt@FontSize}
\newlength{\mt@RightSkip}
\newlength{\mt@TextHeight}
\newlength{\mt@OffsetX}
\newlength{\mt@OffsetY}

\usepackage{eso-pic}
\usepackage{type1cm}
\usepackage{graphicx}

\newcommand{\margintext}[1]{
  \ifx\pdfoutput\undefined\write16{WARNING: Margintext
      will only correctly show up in PS - FILE!}
  \fi
  \AddToShipoutPicture{%
    \setlength{\mt@MarginWidth}{\oddsidemargin}%
    \addtolength{\mt@MarginWidth}{1in}%
    \setlength{\mt@PageHeight}{\paperheight}%
    \setlength{\mt@MaxWidth}{.8\mt@MarginWidth}%
    \setlength{\mt@FontSize}{12mm}%
    \setlength{\mt@RightSkip}{3mm}%
    \setlength{\mt@ActualWidth}{15mm}%
    \ifthenelse{\lengthtest{\mt@ActualWidth > \mt@MaxWidth}}%
    {
      \setlength{\mt@FontSize}{.6\mt@MarginWidth}
      \setlength{\mt@RightSkip}{.2\mt@MarginWidth}
      \setlength{\mt@ActualWidth}{.8\mt@MarginWidth}
    }{}
    \setlength{\mt@OffsetX}{\mt@ActualWidth}
    \setlength{\mt@OffsetY}{0mm}
    \setlength{\unitlength}{1pt}%
    \put(\strip@pt\mt@OffsetX,\strip@pt\mt@OffsetY){%
      \rotatebox{90}
        {
          \makebox[\mt@PageHeight][c]
          {\textcolor[gray]{0.75}{\fontfamily{cmss}
              \fontseries{m}
              \fontshape{n}
              \fontsize{\mt@FontSize}{\mt@FontSize}
              \selectfont{#1}}}
        }
      }
    }
}

%% Collect information from Subversion
% If the file svn_version.tex exists, we will read it, in there
% the command \svnVersion is defined. If the file does not exist, we
% print a warning and set \svnVersion to Unknown
\newboolean{draftmargin}
\setboolean{draftmargin}{false}

\IfFileExists{draft_control.tex}{%
\message{Draft control file exists.}%
\input{draft_control.tex}%
}{% 
\message{ WARNING: draft_control.tex not found.}%
\newcommand{\svnVersion}{???}%
}


\ifthenelse{ \boolean{draftmargin} }
        {
                \margintext{Rev: {\svnVersion}\hspace{1em}Built: {\the\year-\pt@twodigit\month-\pt@twodigit\day} {\printtime}}
        }
        {}

\makeatother



==> extern/layout_commands.tex <==
\usepackage{ifthen}
\usepackage{amsmath}
\usepackage{amsthm}

\makeatletter

\newcommand{\titlefamily}{}%
\newcommand{\thmfamily}{}%
\newcommand{\sectitlefnt}{}%
\newcommand{\subsectitlefnt}{}%
\newcommand{\ps@footnumber}{}

%% Typesetting equations
\renewcommand{\theequation}{\arabic{section}.\arabic{equation}}
\numberwithin{equation}{section}

\newcommand{\fillbox}{\hspace*{\fill}\ensuremath{\Box}}
\renewcommand{\qedsymbol}{\fillbox}

\ifthenelse{\isundefined{\nofancylayout}}
{%
  \renewcommand{\titlefamily}{\sffamily}%
  \renewcommand{\thmfamily}{\sffamily}%
  \renewcommand{\sectitlefnt}{\titlefamily\bfseries\Large}%
  \renewcommand{\subsectitlefnt}{\titlefamily\bfseries}%
  % 
  %% Paper size and margins
  % \usepackage[shiftmargins]{vmargin}
  % \setpapersize{A4}%
  % \setmarginsrb{35mm}{25mm}{30mm}{25mm}{0mm}{0mm}{10mm}{3\baselineskip}%
  %
  \usepackage{calc}
  \usepackage[totalwidth=75ex,totalheight=41\baselineskip,vmarginratio=4:5,footskip=3\baselineskip,hcentering]{geometry}
  
  %% Typesetting the titles
  \renewcommand{\section}{\@startsection%
    {section}%
    {1}%
    {0mm}%
    {-\baselineskip}%
    {\baselineskip}%
    {\sectitlefnt}}%
  \renewcommand{\subsection}{\@startsection
    {subsection}%
    {2}%
    {0mm}%
    {-\baselineskip}%
    {0.5\baselineskip}%
    {\subsectitlefnt}}%
  \renewcommand{\ps@footnumber}{%
    \renewcommand{\@oddhead}{}%
    \renewcommand{\@evenhead}{}%
    \renewcommand{\@oddfoot}{\hfill{\thepage}}%
    \renewcommand{\@evenfoot}{{\thepage}\hfill}}
  \makeatother
  % 
  %% Typesetting Paragraphs
  \setlength{\parskip}{1ex plus .5ex minus 0ex}
  \setlength{\parindent}{0em}
  % 
  %% Typesetting Theorems
  \newtheoremstyle{my_plain}%
  {\parskip}% above skip
  {\parskip}% below skip
  {\normalfont\itshape}% body font
  {}% indent
  {\normalfont\thmfamily\bfseries}% head font
  {.}% headpunct
  { }% headspace
  {}% custom-head-spec
  
  \newtheoremstyle{my_remark}%
  {\parskip}% aboveskip
  {\parskip}% belowskip
  {\normalfont}% bodyfont
  {}% indent
  {\normalfont\thmfamily\bfseries}% headfont
  {.}% headpunct
  { }% headspace
  {}% custom-head-spec
  
  {
    \theoremstyle{my_plain}
    \newtheorem{theorem}{Theorem}[section]
    \newtheorem{proposition}[theorem]{Proposition}
    \newtheorem{corollary}[theorem]{Corollary}
    \newtheorem{lemma}[theorem]{Lemma}
    \newtheorem{definition}[theorem]{Definition}
  }
  
  {
    \theoremstyle{my_remark}
    \newtheorem{remark}[theorem]{Remark}
  }
    
}{%
  \newtheorem{theorem}{Theorem}[section]%
  \newtheorem{proposition}[theorem]{Proposition}%
  \newtheorem{corollary}[theorem]{Corollary}%
  \newtheorem{lemma}[theorem]{Lemma}%
  \newtheorem{definition}[theorem]{Definition}%
  \theoremstyle{remark}%
  \newtheorem{remark}[theorem]{Remark}%
}

\newenvironment{abst}{\begin{quote}\small\thmfamily\bfseries
    Abstract. \normalfont\small}{\end{quote}}


==> inequality.tex <==
\section{A sharp inequality for the area of a strongly stable CMC
  surface}
In this section we will assume that $(M,g)$ has $R_M\geq 0$ in
addition to the existence of an interior boundary $\del M$ which is an
outermost minimal surface. In this setting we can derive a bound on
the area of a strongly stable CMC surface in terms of the mass
$(M,g)$. In order to make the mass well defined we assume that in the
asymptotically flat coordinates
\begin{equation*}
  r |g-\delta|  + r^2 |\nabla - D| \leq C
\end{equation*}
and
\begin{equation*}
  \int_M |\ScalM| \dvol < \infty.
\end{equation*}
In this case we know that the ADM-mass
\begin{equation*}
  m_\mathrm{ADM} : =\lim_{R\to\infty} \frac{1}{16\pi} \int_{\{r=R\}}
  (g_{ij,i} - g_{ii,j} \nu^j \dmu,
\end{equation*}
is a well-defined geometric invariant
\cite{Bartnik:1986}. Furthermore, the Penrose inequality
\cite{Penrose:1973,Huisken-Ilmanen:2001,Bray:2001} states that
\begin{equation*}
  m_\mathrm{ADM} \geq \sqrt{\frac{|\Sigma|}{16\pi}}.
\end{equation*}
Using the inverse mean curvature flow from \cite{Huisken-Ilmanen:2001}
we can show a different lower bound for $\mADM$ involving the area of
a strongly stable CMC surface. The key quantity in this process is the
Hawking mass $m_H(\Sigma)$ of a surface $\Sigma\subset M$,
\begin{equation*}
  m_H(\Sigma)
  =
  \frac{|\Sigma|^{1/2}}{(16\pi)^{3/2}}
  \left( 16\pi - \int_\Sigma H^2 \dmu \right).
\end{equation*}
In the sequel we denote by $R(\Sigma)$ the geometric area radius of
$\Sigma$,
\begin{equation*}
  R(\Sigma) := \sqrt{\frac{|\Sigma|}{4\pi}},
\end{equation*}
so that $|\Sigma| = 4\pi R(\Sigma)^2$. For strongly stable CMC
surfaces we can show the following bound on the area radius.
\begin{lemma}
  If $\Sigma$ is a strongly stable, connected CMC surface in $(M,g)$,
  then
  \begin{equation*}
    R(\Sigma) \leq 3 m_H(\Sigma).
  \end{equation*}
\end{lemma}
\begin{proof}
  The same computation as in the proof of lemma~\ref{thm:curv_bound},
  taking into account that $\ScalM\geq 0$ implies that
  \begin{equation*}
    \int_\Sigma H^2 \dmu \leq \frac{16\pi}{3}.
  \end{equation*}
  In view of the definition of $m_H$ this yields the claim.
\end{proof}
The interesting point now is the possibility to use inverse mean
curvature flow to relate $m_H(\Sigma)$ to $\mADM$.




%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "master"
%%% End: 

